Envisioning the Future of Cyber Security in Post-Quantum Era: A Survey on PQ Standardization, Applications, Challenges and Opportunities

The rise of quantum computers exposes vulnerabilities in current public key cryptographic protocols, necessitating the development of secure post-quantum (PQ) schemes. Hence, we conduct a comprehensive study on various PQ approaches, covering the constructional design, structural vulnerabilities, and offer security assessments, implementation evaluations, and a particular focus on side-channel attacks. We analyze global standardization processes, evaluate their metrics in relation to real-world applications, and primarily focus on standardized PQ schemes, selected additional signature competition candidates, and PQ-secure cutting-edge schemes beyond standardization. Finally, we present visions and potential future directions for a seamless transition to the PQ era.

==> Acknowledgments.tex <==
\section{Acknowledgments}
aaaaaaaaaaaaa

==> Implementation.tex <==
\section{Implementation Analysis}
	The rise of novel computing platforms, such as cloud computing, and
	the Internet of Things (IoT), necessitates the adoption of PQC standards.
	Consequently, it becomes essential to incorporate a wide range of
	cryptographic techniques. However, this is just one aspect of the
	broader picture. At the computing platform level, we observe a varied
	array of computing capabilities, spanning from high-performance virtualized
	environments like cloud computing to resource-limited IoT platforms.
	In the realm of high speed applications which require cryptographic
	implementations that deliver both high performance and energy efficiency
	the challenge lies in designing hardware that can accommodate agility
	in cryptographic operations. Securing IoT devices poses a particular
	challenge due to their reliance on batteries and limited computational
	power and memory resources. This necessitates the development and
	implementation of energy-efficient and lightweight algorithms specifically
	designed for IoT devices. 
	
	In this section, first we summarized the implementation challenges
	which are common in any PQC family for both high speed and low constrained
	devices. Subsequently, we delve into the specific challenges that
	are unique to each PQC family. Lastly, we conduct a comparative analysis
	of the KEM and signature schemes selected as finalists and winners
	in the fourth round of the National Institute of Standards and Technology
	(NIST) post-quantum cryptography competition. The focus of this comparison
	lies in evaluating the implementation aspects of these schemes on
	different platforms, including Desktop computers (pure software),
	Microcontrollers, and FPGA (pure hardware) platforms.
	
	\subsection{Common Implementation challenges}
	
	\subsubsection{Key size limitation}
	
	The advancement of computing and communications technologies has led
	to a significant reduction in the computational effort required to
	break certain asymmetric encryption schemes. As a result, there has
	been a need to increase the recommended minimum key size for these
	schemes to maintain an adequate level of security. Increasing the
	key size can be seen as a temporary solution until technological advancements
	can catch up and provide the necessary computational power. As technology
	progresses, it is expected that the computational effort required
	to break certain asymmetric encryption schemes will decrease, making
	larger key sizes unnecessary for maintaining security. Furthermore,
	constrained IoT devices have a limited memory size and can not benefit
	from this solution. So we should not use PQC schemes which requires
	large public or private keys like McEliece in constrained devices.
	
	\subsubsection{Key generation multiple usage}
	
	Certain post-quantum cryptosystems impose limitations on the number
	of messages that can be signed using the same key in order to prevent
	potential attacks. Consequently, generating new keys for each group
	of signed messages becomes necessary. However, traditional IoT devices
	may face challenges in efficiently managing the computational resources
	required for key generation. This additional overhead can strain the
	limited capabilities of IoT devices. Hence, the performance of the
	key generation component in any cryptographic scheme is crucial and
	should be given equal importance as other parts of the system. 
	
	\subsubsection{Protection from fault and side-channel attacks}
	
	To ensure the robustness of developed and optimized post-quantum cryptosystems,
	it is crucial to assess their physical security, particularly within
	an IoT context. The implementation of the PQC schemes may be vulnerable
	to physical attacks. Attackers may gain physical access to IoT devices
	executing these algorithms, making physical security a significant
	concern. As a result, it becomes imperative to design and evaluate
	the proposed cryptosystems with the objective of mitigating potential
	physical attacks.
	
	\subsection{Type based Implementation challenges}
	
	\subsubsection{Lattice based cryptography}
	
	Lattice-based cryptosystems offer robust security proofs and are known
	for their simplicity and speed of implementation. However, when utilizing
	lattice-based cryptosystems in IoT applications, it becomes necessary
	to apply compression techniques and optimization strategies. This
	is because the key sizes required by lattice-based schemes tend to
	be longer compared to traditional pre-quantum cryptosystems, although
	they are still smaller than those used by code-based or hash-based
	cryptosystems. By employing compression techniques and optimizations,
	the overhead associated with key sizes can be reduced, making lattice-based
	cryptosystems more suitable for resource-constrained IoT environments. 
	
	In the evaluation of components within a Lattice-Based Cryptosystem
	(LBC) that inform the actual implementation, two critical aspects
	stand out. By carefully evaluating and optimizing these critical components,
	the overall performance and security of the LBC can be enhanced, making
	it more suitable for practical applications. Firstly, the polynomial
	multiplication for ideal lattices and matrix multiplication for standard
	lattices are identified as the main bottlenecks that impact the speed
	of the system. Efficient algorithms and optimizations targeting these
	operations are crucial for achieving improved performance in LBC implementations.
	Multiple polynomial multiplication methods is described in Table I.
	
	\begin{table}
		\caption{Polynomial Multiplication Methods}
		
		\centering
		
		\begin{tabular}{ccc}
			\hline 
			\textbf{Method} & \textbf{Complexity} & \textbf{Reference}\tabularnewline
			\hline 
			Schoolbook & $O(n^{2})$ & \cite{key-4}\tabularnewline
			\hline 
			k way Toom-Cook & $O(n^{1.58})$ & \cite{Cook}\tabularnewline
			\hline 
			SchXXX-Strassen & $O(n^{log(2k-1)/logk)})$ & \cite{Sch=0000F6nhage}\tabularnewline
			\hline 
			Karatsuba & $O(n^{1.58})$ & \cite{Karatsuba}\tabularnewline
			\hline 
			Furer & $O(n.logn.2^{O(log^{*}n)})$ & \cite{F=0000FCrer}\tabularnewline
			\hline 
			FFT & $O(n.log^{n})$ & \cite{FFT}\tabularnewline
			\hline 
		\end{tabular}
		
	\end{table}
	
	Secondly, discrete Gaussian sampling plays a vital role in LBCs as
	it is utilized to generate noise that hides the secret information
	within the system. The efficiency and security of the discrete Gaussian
	sampling technique employed are key considerations in the implementation
	of an LBC. The effectiveness of a discrete Gaussian sampler is defined
	by a tuple of three parameters: $\textgreek{sv}$, $\textgreek{l}$, and
	$\textgreek{t}$. Each parameter serves a specific purpose in shaping
	the characteristics of the discrete Gaussian distribution.
	\begin{enumerate}
		\item $\textgreek{sv}$: The standard deviation controls the dispersion of
		data points from the mean. A higher value of $\textgreek{sv}$ results
		in a wider distribution with more spread-out data points, while a
		lower value of $\textgreek{sv}$ leads to a narrower distribution with
		data points clustered closer to the mean.
		\item $\textgreek{l}$: The precision parameter governs the statistical difference
		between an ideal, perfect discrete Gaussian sampler and the implemented
		sampler. It ensures that the implemented sampler approximates the
		ideal behavior with a desired level of accuracy.
		\item $\textgreek{t}$: The distribution tail-cut determines the portion of
		the distribution that is ignored or considered insignificant. By specifying
		a $\textgreek{t}$ value, the sampler excludes data points beyond a certain
		threshold, reducing computational complexity and enabling more efficient
		sampling.
	\end{enumerate}
	Optimizing these parameters allows for fine-tuning the discrete Gaussian
	sampler to meet specific requirements in terms of statistical characteristics,
	computational efficiency, and security considerations within the context
	of the overall lattice-based cryptosystem implementation. Different
	Gaussian samplers are described in Table II. 
	
	\begin{table}
		\caption{Different Gaussian Samplers Referenced From Nejatollahi et al. \cite{Nejatollahi}}
		
		\centering
		
		\begin{tabular}{cccc}
			\hline 
			\textbf{Sampler} & \textbf{Speed} & \textbf{Features} & \textbf{Reference}\tabularnewline
			\hline 
			\multirow{2}{*}{Rejection} & \multirow{2}{*}{slow} & Convenient for  & \multirow{2}{*}{\cite{Rejection_sampler}}\tabularnewline
			&  & constrained devices & \tabularnewline
			\hline 
			\multirow{2}{*}{Ziggurat} & \multirow{2}{*}{flexible} & Convenient for  & \multirow{2}{*}{\cite{Ziggurat}}\tabularnewline
			&  & software implementation & \tabularnewline
			\hline 
			\multirow{2}{*}{CDT} & \multirow{2}{*}{fast} & Convenient for  & \multirow{2}{*}{\cite{CDT}}\tabularnewline
			&  & digital signature & \tabularnewline
			\hline 
			\multirow{2}{*}{Knuth-Yao} & \multirow{2}{*}{fastest} & Not convenient for  & \multirow{2}{*}{\cite{Knuth}}\tabularnewline
			&  & digital signature & \tabularnewline
			\hline 
			\multirow{2}{*}{Bernoulli} & \multirow{2}{*}{fast} & convenient for  & \multirow{2}{*}{\cite{Bernoli}}\tabularnewline
			&  & any scheme & \tabularnewline
			\hline 
			\multirow{2}{*}{Binomial} & \multirow{2}{*}{fast} & Not convenient for  & \multirow{2}{*}{\cite{Binomial}}\tabularnewline
			&  & digital signature & \tabularnewline
			\hline 
		\end{tabular}
	\end{table}
	
	
	\subsubsection{Code based cryptography}
	
	Code-based cryptosystems, such as McEliece's cryptosystem, are based
	on the theory of error-correction codes. Error-correction codes have
	long been used to provide redundancy in digital communications, ensuring
	reliable transmission of data. McEliece's cryptosystem specifically
	relies on binary Goppa codes and utilizes the syndrome decoding problem
	as a basis for its security.
	
	In terms of performance, McEliece's cryptosystem is known for fast
	encryption and reasonably fast decryption. However, one significant
	drawback of implementing this cryptosystem in resource-constrained
	IoT devices is the large size of the public and private keys. The
	key sizes typically range from 100 kB to several megabytes, which
	can be impractical for devices with limited resources.
	
	To address this issue, various compression and decompression techniques
	can be explored. These techniques aim to reduce the size of the keys
	without compromising the security of the cryptosystem. Additionally,
	researchers may propose different versions of the McEliece scheme
	based on alternative codes, which could potentially offer smaller
	key sizes while maintaining an acceptable level of security.
	
	The exploration of compression techniques and alternative code choices
	is an active area of research in code-based cryptography. The goal
	is to make code-based cryptosystems more feasible for implementation
	in resource-constrained devices like IoT devices, without sacrificing
	their security properties. 
	
	The key generation step is the most time consuming operation in McEliece.
	In the McEliece and Niederreiter schemes, the public key is commonly
	randomized by multiplying it with specific matrices. In the case of
	McEliece, the row scrambling is achieved through Gaussian elimination
	instead of matrix multiplication with a non-singular random matrix.
	This process transforms the parity-check matrix into a systematic
	form, which serves as the public key. However, when implementing these
	schemes on embedded devices, the challenge arises from the large size
	of the parity-check matrix, making it difficult to store in memory
	and perform Gaussian elimination efficiently.
	
	\subsubsection{Hash based cryptography}
	
	\subsection{NIST $4^{th}$ round winners and finalist details}
	
	In this section, we depicted and showed the performance of NIST$4^{th}$
	round schemes. We focused on Intel, FPGA, and ARM platforms for the
	evaluation. 
	
	\begin{table}[t]
		\centering
		
		\caption{NIST Security Strength Categories}
		
		\begin{tabular}{cc}
			\hline 
			\textbf{Level} & \textbf{Security Description}\tabularnewline
			\hline 
			1 & At least as hard to break as AES128\tabularnewline
			\hline 
			2 & At least as hard to break as SHA256\tabularnewline
			\hline 
			3 & At least as hard to break as AES192\tabularnewline
			\hline 
			4 & At least as hard to break as SHA384\tabularnewline
			\hline 
			5 & At least as hard to break as AES256\tabularnewline
			\hline 
		\end{tabular}
	\end{table}
	
	\begin{table*}
		\centering
		
		\caption{Comparing Key Size of NIST$4^{th}$ Round KEMs.}
		
		\begin{tabular}{ccccccc}
			\hline 
			\textbf{Scheme} & \textbf{Type} & \textbf{NIST Security Level} & \textbf{Public Key Size} & \textbf{Private Key Size} & \textbf{State} & \textbf{References}\tabularnewline
			\hline 
			Crystal Kyber-512 & Lattice based & 1 & 800 & 1,632 & Winner & \cite{Kyber_Official}\tabularnewline
			\hline 
			Crystal Kyber-512 90s & Lattice based & 1 & 800 & 1,632 & Winner & \cite{Kyber_Official}\tabularnewline
			\hline 
			Crystal Kyber-768 & Lattice based & 3 & 1,184 & 2,400 & Winner & \cite{Kyber_Official}\tabularnewline
			\hline 
			Crystal Kyber-768 90s & Lattice based & 3 & 1,184 & 2,400 & Winner & \cite{Kyber_Official}\tabularnewline
			\hline 
			Crystal Kyber-1024 & Lattice based & 5 & 1,568 & 3,168 & Winner & \cite{Kyber_Official}\tabularnewline
			\hline 
			Crystal Kyber-1024 90s & Lattice based & 5 & 1,568 & 3,168 & Winner & \cite{Kyber_Official}\tabularnewline
			\hline 
			BIKE Level 1 & Code based & 1 & 1,540 & 280 & Round 4 Candidates & \cite{Bike_Official}\tabularnewline
			\hline 
			BIKE Level 3 & Code based & 3 & 3,082 & 418 & Round 4 Candidates & \cite{Bike_Official}\tabularnewline
			\hline 
			BIKE Level 5 & Code based & 5 & 5,121 & 580 & Round 4 Candidates & \cite{Bike_Official}\tabularnewline
			\hline 
			McEliece 348864 & Code based & 1 & 261,120 & 6,492 & Round 4 Candidates & \cite{McEliece_Official}\tabularnewline
			\hline 
			McEliece 6688128 & Code based & 3 & 1,044,992 & 13,932 & Round 4 Candidates & \cite{McEliece_Official}\tabularnewline
			\hline 
			McEliece 8192128 & Code based & 5 & 1,357,824 & 14,080 & Round 4 Candidates & \cite{McEliece_Official}\tabularnewline
			\hline 
			HQC Level 1 & Code based & 1 & 6,170 & 252 & Round 4 Candidates & \cite{HQC_Official}\tabularnewline
			\hline 
			HQC Level 3 & Code based & 3 & 10,918 & 404 & Round 4 Candidates & \cite{HQC_Official}\tabularnewline
			\hline 
			HQC Level 5 & Code based & 5 & 15,898 & 532 & Round 4 Candidates & \cite{HQC_Official}\tabularnewline
			\hline 
			SIKE & Isogeny based & 1 & 330 & 374 & Round 4 Candidates & \cite{SIKE_Official}\tabularnewline
			\hline 
		\end{tabular}
	\end{table*}
	
	\begin{table*}
		\centering
		
		\caption{Comparing The Performance of NIST$4^{th}$ Round KEMs on Intel, ARM,
			and FPGA Platforms.}
		
		\begin{tabular}{cccccccc}
			\hline 
			\multirow{2}{*}{\textbf{Scheme}} & \multirow{2}{*}{\textbf{Platform Architecture}} & \textbf{Performance Evaluation } & \multirow{2}{*}{\textbf{Frequency}} & \multirow{2}{*}{\textbf{Key Generation}} & \multirow{2}{*}{\textbf{Encapsulation}} & \multirow{2}{*}{\textbf{Decapsulation}} & \multirow{2}{*}{\textbf{Reference}}\tabularnewline
			&  & \textbf{Hardware} &  &  &  &  & \tabularnewline
			\hline 
			\multirow{3}{*}{Crystal Kyber-512} & Intel & Intel Core i7-4770K & 3.5 GHz & 122 & 154 & 187 & \cite{Kyber_Official}\tabularnewline
			\cline{2-8} \cline{3-8} \cline{4-8} \cline{5-8} \cline{6-8} \cline{7-8} \cline{8-8} 
			& ARM & Cortex-M4  & 24 MHz & 575 & 763 & 730 & \cite{Kyber_Cortex_M4}\tabularnewline
			\cline{2-8} \cline{3-8} \cline{4-8} \cline{5-8} \cline{6-8} \cline{7-8} \cline{8-8} 
			& FPGA & Xilinx Artix-7  & 161 MHz & 3.8 & 5.1 & 6.7 & \cite{FPGA_Kyber}\tabularnewline
			\hline 
			\multirow{3}{*}{Crystal Kyber-768} & Intel & Intel Core i7-4770K & 3.5 GHz & 199 & 235 & 274 & \cite{Kyber_Official}\tabularnewline
			\cline{2-8} \cline{3-8} \cline{4-8} \cline{5-8} \cline{6-8} \cline{7-8} \cline{8-8} 
			& ARM & Cortex-M4 & 24 MHz & 946 & 1,167 & 1,117 & \cite{Kyber_Cortex_M4}\tabularnewline
			\cline{2-8} \cline{3-8} \cline{4-8} \cline{5-8} \cline{6-8} \cline{7-8} \cline{8-8} 
			& FPGA & Xilinx Artix-7  & 161 MHz & 6.3 & 7.9 & 10 & \cite{FPGA_Kyber}\tabularnewline
			\hline 
			\multirow{3}{*}{Crystal Kyber-1024} & Intel & Intel Core i7-4770K & 3.5 GHz & 307 & 346 & 396 & \cite{Kyber_Official}\tabularnewline
			\cline{2-8} \cline{3-8} \cline{4-8} \cline{5-8} \cline{6-8} \cline{7-8} \cline{8-8} 
			& ARM & Cortex-M4 & 24 MHz & 1,483 & 1,753 & 1,698 & \cite{Kyber_Cortex_M4}\tabularnewline
			\cline{2-8} \cline{3-8} \cline{4-8} \cline{5-8} \cline{6-8} \cline{7-8} \cline{8-8} 
			& FPGA & Xilinx Artix-7  & 161 MHz & 9.4 & 11.3 & 14 & \cite{FPGA_Kyber}\tabularnewline
			\hline 
			\multirow{3}{*}{BIKE Level 1} & Intel & Intel Xeon Platinum & 2.5 GHz & 589 & 97 & 1,135 & \cite{Bike_Official}\tabularnewline
			\cline{2-8} \cline{3-8} \cline{4-8} \cline{5-8} \cline{6-8} \cline{7-8} \cline{8-8} 
			& ARM & Cortex-M4 & 24 MHz & 24,935 & 3,253 & 49,911 & \cite{BIKE_ARM}\tabularnewline
			\cline{2-8} \cline{3-8} \cline{4-8} \cline{5-8} \cline{6-8} \cline{7-8} \cline{8-8} 
			& FPGA & Xilinx Artix-7  & 161 MHz & 187 & 28 & 421 & \cite{Bike_Hardware}\tabularnewline
			\hline 
			\multirow{3}{*}{BIKE Level 3} & Intel & Intel Xeon Platinum & 2.5 GHz & 1,823 & 223 & 3,887 & \cite{Bike_Official}\tabularnewline
			\cline{2-8} \cline{3-8} \cline{4-8} \cline{5-8} \cline{6-8} \cline{7-8} \cline{8-8} 
			& ARM & Cortex-M4 & 24 MHz & 59,820 & 8,376 & 139,234 & \cite{BIKE_ARM}\tabularnewline
			\cline{2-8} \cline{3-8} \cline{4-8} \cline{5-8} \cline{6-8} \cline{7-8} \cline{8-8} 
			& \multirow{1}{*}{FPGA} & Xilinx Artix-7  & 100 MHz & 693 & 80 & 1,198 & \cite{Bike_Hardware}\tabularnewline
			\hline 
			\multirow{2}{*}{McEliece 348864} & Intel & Intel Haswell CPU & 3.1 GHz & 56,705 & 36.4 & 127.14 & \cite{McEliece_Official}\tabularnewline
			\cline{2-8} \cline{3-8} \cline{4-8} \cline{5-8} \cline{6-8} \cline{7-8} \cline{8-8} 
			& ARM & Cortex-M4 & 24 MHz & 1,589,600 & 482.5 & 2,291 & \cite{McEliece_ARM}\tabularnewline
			\hline 
			\multirow{1}{*}{McEliece 6688128} & Intel & Intel Haswell CPU & 3.1 GHz & 443,746 & 171.4 & 306 & \cite{McEliece_Official}\tabularnewline
			\hline 
			\multirow{1}{*}{McEliece 8192128} & Intel & Intel Haswell CPU & 3.1 GHz & 486,195 & 156.9 & 310 & \cite{McEliece_Official}\tabularnewline
			\hline 
			HQC Level 1 & Intel & Intel Core i7-7820 & 3.6 GHz & 200.5 & 383.8 & 508.9 & \cite{HQC_Official}\tabularnewline
			\hline 
			HQC Level 3 & Intel & Intel Core i7-6700 & 3.6 GHz & 403.3 & 765.1 & 983.6 & \cite{HQC_Official}\tabularnewline
			\hline 
			HQC Level 5 & Intel & Intel Core i7-6700 & 3.6 GHz & 651.4 & 1,257.1 & 1,618.3 & \cite{HQC_Official}\tabularnewline
			\hline 
			SIKE & Intel & Intel Core i7-6700 & 3.4 GHz & 1,047,991 & 1,482,681 & 1,790,304 & \cite{SIKE_Official}\tabularnewline
			\hline 
		\end{tabular}
	\end{table*}
	\begin{figure}
		
		\includegraphics[width=1\columnwidth]{Figures/KEM_ARM_Codebased}
		
		\caption{The time required for encapsulation, decapsulation, and key generation
			for Code based schemes on NIST's$4^{th}$round KEMs, implemented on
			ARM platform.}
	\end{figure}
	\begin{figure}
		\includegraphics[width=1\columnwidth]{Figures/KEM_ARM_Lattice}
		
		\caption{The time required for encapsulation, decapsulation, and key generation
			for Lattice based schemes on NIST's$4^{th}$round KEMs, implemented
			on ARM platform.}
	\end{figure}
	\begin{figure}
		\includegraphics[width=1\columnwidth]{Figures/KEM_Intel_Codebased}
		
		\caption{The time required for encapsulation, decapsulation, and key generation
			for Code based schemes on NIST's$4^{th}$round KEMs, implemented on
			Intel platform.}
		
	\end{figure}
	\begin{figure}
		\includegraphics[width=1\columnwidth]{Figures/KEM_Intel_Lattice}
		
		\caption{The time required for encapsulation, decapsulation, and key generation
			for Lattice based schemes on NIST's$4^{th}$round KEMs, implemented
			on Intel platform.}
		
	\end{figure}
	\begin{figure}
		\includegraphics[width=1\columnwidth]{Figures/KEM_Scatter_ARM}
		
		\caption{The relation between key size and decapsulation time for schemes on
			NIST's$4^{th}$round KEMs, implemented on ARM platform. }
		
	\end{figure}
	\begin{figure}
		
		\includegraphics[width=1\columnwidth]{Figures/Signature_Arm_HashBased}
		
		\caption{The time required for signing, verifying, and key generation for Hash
			based schemes on NIST's$4^{th}$round signatures, implemented on ARM
			platform. }
		
	\end{figure}
	\begin{figure}
		\includegraphics[width=1\columnwidth]{Figures/Signature_Arm_Lattice}
		
		\caption{The time required for signing, verifying, and key generation for Lattice
			based schemes on NIST's$4^{th}$round signatures, implemented on ARM
			platform. }
		
	\end{figure}
	\begin{figure}
		
		\includegraphics[width=1\columnwidth]{Figures/Signature_Intel_HashBased}\caption{The time required for signing, verifying, and key generation for Hash
			based schemes on NIST's$4^{th}$round signatures, implemented on Intel
			platform. }
		
	\end{figure}
	\begin{figure}
		
		\includegraphics[width=1\columnwidth]{Figures/Signature_Intel_Lattice}
		
		\caption{The time required for signing, verifying, and key generation for Lattice
			based schemes on NIST's$4^{th}$round signatures, implemented on Intel
			platform. }
		
	\end{figure}
	\begin{figure}
		\includegraphics[width=1\columnwidth]{Figures/Signature_Scatter}
		
		\caption{The relation between key size and signing time for schemes on NIST's$4^{th}$round
			signatures, implemented on ARM platform. }
	\end{figure}

==> Preliminaries.tex <==
\section{Exhaustive Study of PQ Standardizations and Metrics}
\label{section2}

Within this section, our objective is to comprehensively study worldwide initiatives focused on PQC standardization, along with the various projects and institutions that prioritize PQC.
In addition to this examination, we will delve into the standardization prerequisites and evaluation metrics that facilitate the transition from the pre-quantum to the post-quantum era, establishing a foundation for this shift.

%--------------------------------------------------
%  Standardization
%--------------------------------------------------
\subsection{PQC Standardizations and Procedures}
The standardization process plays a significant role in facilitating the transition to a new cybersecurity infrastructure. With the advent of quantum computers, various countries, institutions, and organizations are actively engaged in global efforts to standardize, develop, and implement PQC. In this part, we aim to illustrate the comprehensive scope of these standardization initiatives, ongoing projects, and the most recent discoveries and progress associated with them.

Despite the extensive historical background of PQC research and development, it was not until 2006 that the inaugural PQCrypto conference, dedicated exclusively to PQC, was held on an international scale.
%They have held more than 13 successful conferences. PQCRYPTO aims to develop a diverse range of post-quantum public-key systems with high security, optimize their performance for various platforms such as mobile devices, the cloud, IoT, and deliver efficient implementations for real-world applications.
NIST assumes a prominent and dynamic role in global cybersecurity practices, as evidenced by its involvement in standardizing widely utilized cryptographic components such as the AES algorithm and SHA hash functions. 
Functioning as the primary authority for standardizing PQ primitives, NIST has successfully conducted two competitions. 
The stateful hash-based signature (HBS) competition has concluded, and IETF has published RFCs pertaining to these signatures. 
%Importantly, it is worth noting that these HBS solutions offer robust security guarantees while minimizing the reliance on strong assumptions.
Given the intricacies involved in standardizing PQC compared to symmetric primitives, the transition from PKC to PQC is anticipated to be a time-consuming process, necessitating multiple rounds of analysis. 
This is due to factors such as the diverse range of PQC approaches, algorithms, and the associated implementation costs. 
In light of these considerations, it became imperative to initiate a global competition at the earliest opportunity. 
Consequently, on December 2016, NIST issued a call for PQC standardization, seeking the development of cryptographic algorithms, including PKE schemes, KEMs, and digital signature schemes that offer security against classical as well as quantum computers \cite{alagic2022status}.
%===================================================
% The folowwing paragraph can be completely removed
%===================================================

%In November 2017, a total of 82 candidate algorithms were submitted, with 5 subsequently withdrawing their entries. Of the remaining 77 submissions, 69 satisfied the minimum requirements and were accepted, encompassing 20 digital signatures and 49 PKEs or KEMs.
%During the first round, the criteria for acceptance were primarily focused on "complete and proper submission," with other factors such as implementation, cryptanalysis, and performance costs temporarily set aside. 
%In January 2019, NIST advanced 26 algorithms to the second round, comprising 17 PKE or KEMs and 9 digital signatures. 
%The criteria for this round were based on defined security considerations, cost and performance factors, as well as implementation characteristics. 
%By July 2022, the candidate algorithms were announced, revealing 7 finalists, consisting of 4 PKE or KEMs and 3 signature schemes. Additionally, there were 8 alternative schemes, comprising 5 PKE/KEMs and 3 digital signatures. 
%The selection of these schemes was based on in-depth security analyses, with the majority claiming to meet Category 5 security requirements. Performance considerations such as key sizes, computational costs, RAM and gate counts, performance characteristics, detailed implementation specifics, simplicity, and other relevant factors were taken into account.
For more information on each round of NIST's competitions, refer to their reports \cite{alagic2019status,moody2020status,alagic2022status,turan2023status}.
%Following the announcement of the selected schemes for standardization, which included CRYSTALS-Kyber for KEM and CRYSTALS-Dilithium, FALCON, and SPHINCS+ for digital signatures, there were four remaining KEM schemes to be considered in the fourth round. However, no signatures remained for further evaluation. It is worth noting that, apart from SPHINCS+, the digital signatures in the final rounds were predominantly based on the hardness of structured lattices.
%))))))))))))))))))))))))))))))))))))))))))))
%To promote diversity in PQC standards, NIST initiated an additional competition, specifically focusing on general-purpose digital signatures for PQC standardization. The call for submissions 
%set a deadline of June 1st, 2023, and 
%emphasized the need for non-lattice algorithms suitable for applications like certificate transparency. A total of 50 schemes from 28 countries have been submitted for this competition, with the required criterion being the proposal of a "short signature and fast verification" solution. 
To promote diversity in PQC standards, NIST initiated an additional competition, specifically focusing on general-purpose digital signatures for PQC standardization. The call for submission emphasized the need for non-lattice algorithms suitable for applications like certificate transparency. The predominant necessary condition is to offer a solution that demonstrates "quick verification and concise signature" properties, capable of accommodating message sizes up to $2^{63}$ bits. Lattice-based proposals must not only ensure EUF-CMA security but also provide additional features beyond Dilithium \cite{ducas2018crystals} and FALCON  \cite{fouque2019fast}. On the other hand, non-lattice proposals must exhibit notable performance benefits over SPHINCS+ \cite{bernstein2019sphincs+}. Notably, NIST has recently disclosed the initial-round schemes in this competition, which will be thoroughly assessed based on each unique approach in the next section \cite{NISTsigCompetition}. 
%)))))))))))))))))))))))))))))))))))))))))
%In addition, NIST collaborates with various agencies, institutions, and entities, such as the National Cybersecurity Center of Excellence (NCCoE), to facilitate the development of tools and proofs of concept aimed at simplifying the transition to PQC. 
Notably, other standardization bodies including ISO, ETSI, and IETF largely rely on NIST to conclude the competition, allowing them to proceed with their respective tasks securely. Besides the standardization entities, all different working groups worldwide involved in the PQC standardization process with their projects and products are depicted in Table \ref{tab:standardization}. 
%The IETF is primarily dedicated to the standardization process of PQC through the establishment of multiple groups with distinct objectives.
%Although the IETF does not introduce new cryptographic designs for PQC, its focus lies in the standardization efforts. In particular, the IETF has undertaken the task of integrating PQC secure schemes into various protocols such as TLS, internet key exchange, and OpenPGP. Furthermore, 
%The IRTF (Internet Research Task Force), functioning as the research branch of the IETF, 
%is making significant progress in finalizing the standardization of hash-based signature algorithms. 
%The IETF 
%has established HBS standards, which encompass the Leighton-Micali signature (LMS) scheme, the eXtended Merkle signature scheme (XMSS), and various multitree variants. 
%To disseminate these standards, the IETF has published stateful HBS RFCs.
%These RFCs serve as documents that outline proposals and specifications, and they are widely embraced by industry participants, although they hold an informal status as standards. 
%Additionally, the working group named Post-Quantum Use In Protocol (PQUIP) focuses on scrutinizing PQ-related concerns from an engineering and operational perspective, without specifically addressing standardization. In parallel, the 3GPP project is dedicated to exploring the implications of quantum technology on cellular networks. Overall, all groups within the IETF share a common objective of integrating PQC algorithms into contemporary protocols, ensuring the seamless incorporation of PQ security measures.

%ETSI (European Telecommunications Standards Institute) actively engages in the standardization process of quantum-resistant communication technologies, with dedicated working groups focused on QKD and PQC. Notably, ETSI has strategically devised and delivered numerous papers, seminars, and workshops pertaining to the standardization of PQC, QKD systems, and quantum communication networks. The organization has also played a crucial role in coordinating technical events in collaboration with reputable institutions such as the Institute for Quantum Computing (IQC) and the ETSI Industry Specification Group (ISG). Since 2015, ETSI has released multiple whitepapers with a specific focus on secure implementations of QKD, quantum-safe cryptography, and the analysis of robust PQC algorithms and associated challenges. The Quantum Safe Cryptography (QSC) working group within ETSI concentrates on algorithms, their practical implementation, and design considerations, with a strong emphasis on real-world and industrial deployment aspects. The group does not introduce new cryptographic primitives but rather provides valuable insights into algorithmic choices and practical deployment strategies. ETSI is actively assuming a proactive stance in establishing the standards for PQC and providing assistance to other international groups and projects in selecting appropriate schemes for secure technological advancements in the PQ era. In pursuit of this objective, ETSI has put forth migration strategies and offered suggestions for diverse applications and scenarios.

%From 2015 onward, the United States National Security Agency (NSA) has been dedicated to transitioning towards PQC and QKD in order to offer secure data transmission solutions for National Security Systems. However, the agency has imposed restrictions on their usage until robust and reliable solutions are made available. The NSA has actively published numerous papers on quantum-resistant algorithms that hold the utmost significance for military and intelligence operations. Furthermore, the NSA has undertaken the task of enhancing the Commercial National Security Algorithm Suite (CNSA) to its latest iteration, version 2.0. This updated version includes a comprehensive set of algorithms for various purposes such as software and firmware signing, PKE, and ensuring a well-coordinated and timely transition process.

%The European Union Agency for Cybersecurity, known as ENISA, has presented a comprehensive overview of the standardization process for PQC. Additionally, ENISA has released multiple newly published reports that focus on the integration of PQC into existing protocols. These reports also explore the utilization of double encryption or double signature techniques within various systems.

%PROMETHEUS, a project funded by the European Union, aims to develop Privacy-Preserving PQ Systems that ensure confidentiality, security, and privacy protection. This project utilizes advanced cryptographic mechanisms, including MPC, Functional Encryption, Homomorphic Encryption, and sophisticated use cases and applications in the PQ era. The primary focus of PROMETHEUS is on leveraging lattice-based cryptography to achieve its objectives.

%The FutureTPM project, funded by the European Union, is dedicated to the development of a Quantum-Resistant Trusted Platform Module (QR TPM). This project places emphasis on ensuring long-term security by addressing the challenges posed by quantum computing. It aims to incorporate run-time risk assessment and create an implementation environment that encompasses hardware, software, and virtual TPM. The goal is to enhance the security and resilience of TPMs against potential threats arising from advancements in quantum computing technology.

%ANSSI, the national cybersecurity authority in France, assumes the role of providing advisory services and regulatory oversight in the field of post-quantum secure cryptographic primitives, even though it is not a standardization agency for their design and development. ANSSI issues various publications concerning the selected PQC schemes, oversees the implementation of security labels, and conducts evaluations of certificates in accordance with European guidelines.

%The FLOQI project, known as the Full-Lifecycle Post-Quantum initiative, receives funding from the German government and collaborates with ESCRYPT to achieve its objective of developing a quantum-resistant public key infrastructure. The anticipated implementation of this infrastructure is envisaged within the domains of Industry 4.0, the automotive industry, and the financial sectors [reference].

%The QuantumRISC project, originating from Germany, specifically addresses the domain of PQC on embedded devices characterized by resource constraints, low power consumption, minimal memory requirements, and stringent security considerations in the PQ era. Furthermore, the project's primary emphasis lies in the practical implementation aspects, encompassing the development of hardware accelerators and software libraries tailored for such constrained devices, targeting real-world industrial scenarios and use cases.

%KBLS, which stands for Kryptobibliothek Botan für langlebige Sicherheit (Botan cryptolibrary for durable security), is a German project that aims to enhance cryptographic libraries for long-term security and provide accessible processes for software developers. This initiative focuses on improving the durability of cryptographic solutions and facilitating their integration into software development practices.

%The Aquorypt research project, originating from Germany, focuses on the scrutiny of quantum-resistant cryptographic processes and their applicability in various software and hardware implementations. As implied by its name, the project specifically investigates the feasibility and considerations associated with implementing PQC algorithms. The project's application area encompasses two main domains. Firstly, it targets industrial embedded systems that possess multiple constraints. Secondly, it addresses the requirements of industrial control systems, such as smart cards, which necessitate high levels of security while operating with limited storage and computational power resources.

%The PQC4MED project, located in Germany, is primarily centered around medical technology, services, and products. As implied by its name, the project's main objective is to explore the utilization of post-quantum secure algorithms within embedded systems, both in terms of hardware and software. The project specifically aims to adopt a security-by-design approach, ensuring PQ security by incorporating hardware secure elements.

%The QuaSiModO project, which receives funding from the German government, has the objective of delivering secure networking solutions. Its primary focus lies in addressing security aspects, feasibility, and implementation considerations across various layers of the VPN network within the PQ era.

%The MTG Enterprise Resource Security (ERS) group is dedicated to the implementation of PQC, the application of PQC solutions, and the integration of PQC into customer applications. Additionally, MTG places significant emphasis on a concept known as crypto-agility, which pertains to the ability to easily incorporate or remove cryptographic algorithms from a product with minimal expenses, effort, and time requirements.

%The CRYPTREC (Cryptography Research and Evaluation Committees) project, supported by the Japanese government, has been undertaking extensive research to assess the security of different ciphers and cryptographic modules. Since 2017, a key focus of their work has been on the security aspects of PQC approaches. As part of their efforts, they have developed a lattice-based scheme called LOTUS, aimed at achieving PQC security. This scheme was also submitted for consideration in the NIST's standardization competition. Despite introducing the concept of versatility, which addresses the overall security of a cryptosystem that combines multiple cryptographic techniques, LOTUS did not advance to the second round of the competition after being rejected.

%The CryotMathCREST project, funded by the Japanese government, focuses on the mathematical aspects, security evaluation, and application considerations of PQ secure cryptosystems. It aims to design a new and innovative model in the field of industrial mathematics and PQC. The project has made significant contributions through the publication of valuable papers and books, as well as organizing conferences and workshops related to this field.

%The Chinese Association for Cryptography Research (CACR), organized a PQC standardization competition exclusively open to Chinese developers and designers from 2018 to 2020. This competition mirrored NIST's efforts and focused on encryption, key agreement, and signature schemes. 
%However, unlike NIST's competition that featured five security categories, CACR's competition only had two security categories: 128-bit and 256-bit.
%In total, the competition received 36 submissions. Among these submissions, three algorithms emerged as the winners, four were placed second, and six secured the third place. 
%Notably, all three prize-winning algorithms were based on lattice-based cryptography. The winning algorithms included the Aigi-Sig signature scheme, the LAC encryption scheme, and the Aigi-Enc encryption scheme. 
%It is worth mentioning that the LAC encryption scheme also participated in NIST's competition and advanced to the second round. However, due to the discovery of multiple attacks, it did not progress to the third round of the NIST competition. 
%Apart from the LAC cryptosystem, Chinese developers submitted two additional schemes to the NIST competition. 
%These schemes, named LPN-based KEMs with Post Quantum Security (Lepton) and Key Consensus from Lattice (KCL), did not advance beyond the first round in the NIST competition.

%Recognizing that the previous Chinese PQC competition was limited to domestic designers and not a global initiative like those conducted by Western countries, there is a strong desire within China to organize an international competition at the ISO (International Organization for Standardization) level for the standardization of their own PQC scheme, adhering to real-world standards. The intention is to commence the commercial migration to PQC by 2025.

%In addition to the efforts focused on PQC standardization, Chinese cryptographic groups have conducted various cryptoanalyses on candidates proposed by NIST for standardization. This includes the examination of schemes such as DRS Signature, HK17 cryptosystem, and compact-LWE scheme.

%Overall, the QApp team in China remains highly engaged in the field of PQC and is actively developing and refining Chinese-designed cryptosystems with the aim of making them practical and applicable. The team responsible for the Quality Assurance Project Plan (QAPP) is currently engaged in the development of a PQLR library. This library incorporates advanced cryptographic algorithms that are resistant to quantum attacks and is integrated into the OpenSSL library for seamless integration with various applications. Additionally, the team is actively working on Qtunnel, a client-server application designed to facilitate secure data transfer in the quantum era. Qtunnel relies on the PQLR Software Development Kit (SDK) and utilizes the NIST's PQC algorithms.

\begin{table*}
	\caption{A Comprehensive analysis of standardization procedures and projects around the world}
	\vspace{-3mm}
	\label{tab:standardization}
	\begin{tabular}{c|c|c|l}
		\toprule
		Project & Country & Focus & Work, Actions, and Products \\
		\midrule		
		IETF \cite{IETF} & Inter & \small{PQC Standardization} & \small{Integrating PQC schemes into many protocols}\\
		& national & \small{Publishing RFCs} & \small{PQUIP works on engineering aspects of PQ}\\
		& & & \small{3GPP works on cellular networks}\\
		\midrule
		ETSI \cite{ETSI} & Europe & \small{PQC \& QKD} & \small{Working groups collaboration: IQC, ISG, QSC}\\
		&  & \small{Standardization} & \small{Publications, seminars, \& whitepapers}\\
		& & & \small{Real-world and industrial PQC development}\\
		& & & \small{Put forth migration strategies \& scenarios}\\
		\midrule
%		ISO [] &  & Standardization & Publishing reports\\
%		\midrule
		NSA \cite{NSA} & USA & \small{Transition towards} & \small{Publishing numerous reports}\\
		& &\small{PQC \& QKD} & \small{PQC in military and intelligence operations}\\
		\midrule
		ENISA \cite{ENISA} & Europe & \small{Standardization Process} & \small{Publishing reports}\\
		& & & \small{Utilization of double encryption/signature}\\		
		\midrule
		PROMETHEUS \cite{FutureTPM} & Europe & \small{Privacy-Preserving PQ Systems} & \small{Ensuring confidentiality and privacy}\\
		& & \small{Lattice-based Cryptography} & \small{Using advanced mechanisms like MPC \& FHE}\\
		\midrule
		FutureTPM \cite{FutureTPM} & Europe & \small{Quantum-Resistant Platform} & \small{Ensuring long-term security in QC}\\
		& & & \small{Risk assessment of run-time, HW \& SW}\\
		\midrule
		ANSSI \cite{ANSSI} & France & \small{Advisory Services} & \small{PQC publications \& evaluation of}\\
		& & \small{Regulation Oversight} & \small{certificates with European guidelines}\\
		\midrule
		FLOQI \cite{FLOQI} & Germany & \small{Full-lifecycle PQC Schemes} & \small{Developing and implementing PKE for }\\
		& & & \small{automotive industry \& financial sectors}\\
		\midrule
		QuantumRISC \cite{koskesh} & Germany & \small{PQC on Embedded Devices} & \small{Practical implementation \& HW development}\\
		& & & \small{for industrial resource constraints devices} \\
		\midrule
		KBLS \cite{KBLS} & Germany & \small{Long-term Security} & \small{Enhancing cryptographic libraries}\\
		& & & \small{Facilitating and development of SW}\\
		\midrule
		Aquorypt \cite{Aquacrypt} & Germany & \small{PQC Implementation} & \small{Implementing on HW \& SW}\\
		 & & & \small{Targets industrial embedded \& control systems}\\
		 & & & \small{with constrained devices like smart cards}\\		
		\midrule
		PQC4MED \cite{PQC4MED} & Germany & \small{Medical Technology Services} & \small{Security approaches for embedded systems}\\
		 & & & \small{By utilizing HW \& SW elements}\\
		\midrule
		QuaSiModO \cite{Qua} & Germany & \small{PQ Secure VPNs} & \small{Delivering secure networking solutions}\\		
		\midrule
		MTG-ERS \cite{MTG} & Germany & \small{PQC Implementation} & \small{Integration of PQC into customer applications}\\
		 & & & \small{Introducing crypto-agility} metric\\
		\midrule 
		CRYPTREC \cite{CRYPTREC} & Japan & \small{Security of approaches} & \small{A lattice-based scheme called LOTUS}\\
		 & & &\small{Introducing the versatility metric}\\
		\midrule
		CryotMathCREST \cite{CryptoMathCREST} & Japan & \small{Mathematical aspects} & \small{Designing an innovative model}\\
		 &  & \small{PQC Cryptosystems' Security} & \small{in industrial mathematics.}\\		
		\midrule
%		CACR [] & China && \\
%		\midrule
		QAPP \cite{CACR} & China & \small{Designing and refining} & \small{Development of PQ libraries}\\
		& & \small{cryptosystems} & \small{Secure data transfer in client-server Apps}\\		
		\midrule
		CACR \cite{CACR} & China & \small{PQC Standardization} & \small{Design Lattice-based Cryptosystems:}\\
		& & \small{Organizing PQC Competition} & \small{LAC, LPN, Lepton, Aigi (Sig/Enc)}\\
		& &  & \small{Performing Cryptanalysis}\\		
		\bottomrule
	\end{tabular}
\end{table*}



%=============================================================
%                Standardization Metrics
%=============================================================

\subsection{Standardization Requirements and Evaluation Metrics}
Here, we present the formal concepts and requirements established by standardization entities. Notably, NIST's standardization efforts encompass clearly defined metrics across three key aspects: security, implementation-cost, and algorithmic characteristics. On the other hand, other standardization organizations and projects predominantly establish application-specific criteria or regulations rather than metrics. 

%\vspace{-2mm}
\textbf{\textit{SECURITY:}}
The main criterion for consideration is undeniably the level of security achieved. NIST has established five security levels based on symmetric key cryptographic primitives that have already been standardized. These levels can be summarized as follows: level one corresponds to breaking AES-128, level two entails finding a collision on a 256-bit hash function (such as SHA2-256 or SHA3-256), level three involves breaking a 192-bit block cipher (AES-192), level four relates to finding a collision on a 384-bit hash function (SHA-384), and level five encompasses a key search on a 256-bit block cipher (AES-256). While the primary focus of the NIST competition is on the first three levels, the submission of parameter sets for level five is also encouraged. 
Apart from achieving these security levels, additional security properties including forward/backward security \cite{yavuz2022frog}, backward compatibility, resistance against attacks like side-channel and multi-key attacks, as well as resistance to misuse are also of importance\cite{alagic2019status}. 

It should be noted that both of the theoretical models such as the Random Oracle Model (ROM) and its extension, the Quantum Random Oracle Model (QROM), involve the capability to respond to queries and provide public accessibility. However, the QROM diverges by permitting quantum adversaries and facilitating quantum operations. 
Technically, for PKE/KEM, they need to demonstrate IND-CPA, IND-CCA, and IND-CCA2 security for general-purpose and ephemeral use cases. On the other hand, signature schemes are expected to provide EUF-CMA security \cite{alagic2022status}.
%Within the realm of cryptography, i
%Also, it is imperative to establish precise definitions for theoretical models such as the Random Oracle Model (ROM) and its extension, the Quantum Random Oracle Model (QROM). Both of these models involve the capability to respond to queries and provide public accessibility. However, the QROM diverges by permitting quantum adversaries and facilitating quantum operations. 

%\vspace{-3mm}
\textbf{\textit{COST, PERFORMANCE, \& IMPLEMENTATION:}}
The costs encompass various factors such as the size of keys, ciphertexts, and signatures, while also considering limitations on memory usage and code size. Furthermore, the evaluation of performance examines the efficiency of computational costs, the intensity of communication, and the rate of decryption failures. Both algorithmic and implementation characteristics are taken into account, including the chosen platform, software effectiveness, and hardware requirements. 
%Advancements in computing and communications have reduced the effort to break asymmetric encryption, necessitating larger key sizes. However, this is a temporary solution until technology catches up. As computing power increases, larger keys will become unnecessary. Constrained IoT devices cannot benefit from larger key sizes.
Besides, the performance of the key generation component is vital and should be prioritized alongside other aspects of the system.
PQ cryptosystems often restrict the number of messages that can be signed with the same key, necessitating key generation for each message group. However, IoT devices may struggle with the computational resources required for key generation, leading to additional overhead and strain on their limited capabilities. 

\textbf{\textit{ATTACK RESISTANCE:}}
%To ensure the robustness of developed and optimized PQ cryptosystems, it is crucial to assess their physical security, particularly within an IoT context. The implementation of the PQC schemes may be vulnerable to physical attacks. Attackers may gain physical access to IoT devices executing these algorithms, making physical security a significant concern. As a result, it becomes imperative to design and evaluate the proposed cryptosystems with the objective of mitigating potential physical attacks.
Rather than mathematically analyze a protocol, side-channel attacks (SCA) target on exploiting vulnerabilities in its implementation to acquire sensitive data. This means that even schemes with security proofs, can still be vulnerable to SCAs. In an SCA, the internal circuits are observed during cryptographic computations, and this information can later be used to extract sensitive data. The process of conducting an SCA involves two crucial steps: gathering the leaked information and turning them into vectors, and searching through the different inputs which result into those leaked information to retrieve the secret value. SCAs can be carried out using various methods, such as those based on acoustics, light, timing, power analysis, and electromagnetic emissions \cite{SCA1,SCA2}, and \cite{SCA3}. The primary distinction between these methods lies in the type of data being analyzed. 

%Good DATA
%%%%%%%%%%%For instance, power analysis attacks involve collecting power traces of a device during different operations over time, whereas timing attacks focus on investigating the time spent on each operation. Among these methods, due to their implementation simplicity and high effectiveness, power, timing, and electromagnetic based attacks are the most common types. 

Fault injection attacks are another type of side channel attacks where errors and faults are deliberately introduced into an algorithm to disrupt its intended operation. The purpose of these attacks is to manipulate the system in such a way that it reveals sensitive data through its unintended leakages. It is crucial to mention that even a single faulty input can have severe consequences on the algorithm's output \cite{SCA4}. 
%Moreover, if the erroneous output is subsequently used as input in other components of the system, it can trigger a chain reaction, impacting the entire system. Therefore, it is crucial to identify and address these faults early on, especially in applications that are costly or involve critical safety considerations \cite{SCA4}.

\textbf{\textit{DIVERSITY:}}
The necessity for alternative candidates and approaches in a standardization process is apparent from the perspective of common sense. Furthermore, when selecting a scheme for standardization from various existing approaches, a significant factor to consider is the diversity metric, which measures variations in mathematical complexity, security assumptions, and algebraic structure. This metric ensures the prevention of a single vulnerability that could compromise global security and undermine the efforts of standardization \cite{alagic2022status}. 

\textbf{\textit{VERSATILITY:}}
The principle behind the versatility metric is rooted in the understanding that a chain is only as strong as its weakest link. This metric aims to assess the security of an entire system when multiple cryptographic primitives are integrated together. While the individual security of each primitive holds significance, the versatility metric highlights the practical application and mathematical proof of their collective utilization. This is relevant as these cryptographic techniques often operate within a system that encompasses various cryptographic components.

\textbf{\textit{EXOTIC FEATURES:}}
While standardization entities primarily concentrate on cryptographic primitives for general-purpose use cases, it is crucial to avoid overlooking the easement of future transition to PQC, the current diverse range of application use cases, and the potential to support exotic features like blind/group/ring signatures, FHE, MPC, SS, etc., and advanced enhancements within these primitives. 

\textbf{\textit{SIMPLICITY \& UNIQUENESS:}}
Besides the aforementioned metrics, there exist certain implicit concepts that lack quantifiable measurements, such as uniqueness, simplicity, and elegance. While standardization entities have not explicitly defined these metrics, they have not been grounds for significant disqualification of schemes either. However, considering these metrics can contribute to a more well-rounded standardization process amidst the wide array of PQC schemes. Specifically, uniqueness, simplicity, and elegance pertain to having a transparent design, minimal reliance on complex mathematical techniques, fewer security assumptions and reductions, and adherence to simpler principles. 


%Kasra
%\subsubsection{Key size limitation}
%Advancements in computing and communications have reduced the effort to break asymmetric encryption, necessitating larger key sizes. However, this is a temporary solution until technology catches up. As computing power increases, larger keys will become unnecessary. Constrained IoT devices cannot benefit from larger key sizes.
%The advancement of computing and communications technologies has led to a significant reduction in the computational effort required to break certain asymmetric encryption schemes. As a result, there has been a need to increase the recommended minimum key size for these schemes to maintain an adequate level of security. Increasing the key size can be seen as a temporary solution until technological advancements can catch up and provide the necessary computational power. As technology progresses, it is expected that the computational effort required to break certain asymmetric encryption schemes will decrease, making larger key sizes unnecessary for maintaining security. Furthermore, constrained IoT devices have a limited memory size and can not benefit from this solution. So we should not use PQC schemes which requires large public or private keys like McEliece in constrained devices.
%\subsubsection{Key generation multiple usage}
%Post-quantum cryptosystems often restrict the number of messages that can be signed with the same key, necessitating key generation for each message group. However, IoT devices may struggle with the computational resources required for key generation, leading to additional overhead and strain on their limited capabilities. Therefore, the performance of the key generation component is vital and should be prioritized alongside other aspects of the system.
%Certain post-quantum cryptosystems impose limitations on the number of messages that can be signed using the same key in order to prevent potential attacks. Consequently, generating new keys for each group of signed messages becomes necessary. However, traditional IoT devices may face challenges in efficiently managing the computational resources required for key generation. This additional overhead can strain the limited capabilities of IoT devices. Hence, the performance of the key generation component in any cryptographic scheme is crucial and should be given equal importance as other parts of the system. 
%\subsubsection{Protection from fault and side-channel attacks}
%To ensure the robustness of developed and optimized post-quantum cryptosystems, it is crucial to assess their physical security, particularly within an IoT context. The implementation of the PQC schemes may be vulnerable to physical attacks. Attackers may gain physical access to IoT devices executing these algorithms, making physical security a significant concern. As a result, it becomes imperative to design and evaluate the proposed cryptosystems with the objective of mitigating potential physical attacks.


%Saeed
%%% intro of side channel







==> Side-channel.tex <==
	\section{Side Channel Analysis }
	
	Rather than mathematically analyze a protocol, side-channel attacks
	(SCA) target vulnerabilities existing in the implementation of it
	to obtain sensitive data. In other words, a scheme may have security
	proofs, but still suffer from SCA. In SCA the internal circuits are
	observed during cryptographic computations and can be exploitet later
	to obtain sensitive information. The two important steps of SCA are
	gathering the leaked information and turning them into vectors, and
	searching through all the secret information that would lead into
	those leaked information until the secret value is found. As a result,
	the noisier and more complex the leaked data, the more difficult to
	perform SCA on them. SCA can be performed through various methods
	such as acoustic based, light based, timing based, power analysis
	based, and electromagnetic emission based \cite{SCA 1,SCA 2,SCA 3,SCA 4,SCA 5},
	and \cite{SCA 6}. The main difference between these methods is related
	to which type of the data is being analyzed. For example, in power
	analysis attacks, the power traces of the device while computing different
	operations over time is collected, while in timing attacks, the spent
	time on each operation is investigated.
	
	Among these methods, due to their implementation simplicity and high
	effectiveness, power, timing, and electromagnetic based attacks are
	the most common types.
	
	Fault injection attacks are another type of side channel attacks that
	inject errors and faults into the algorithm and disrupt its normal
	functionality in a way to force the system to expose sensitive data
	that are collectible from its leakages. In some cases, even a single
	faulty input could have devastating effect on the output of the algorithm.
	Furthermore, if the faulty output is again used in other parts of
	the system as input, the whole system would be effected by a chain
	reaction. Hence, early detection of these faults is essential especially
	in high-cost and safely- critical applications. Fault detection algorithms
	are introduced to prevent such attacks \cite{FA 1} and \cite{Fault detec}. 
	
	Beside these types of SCA, there is another type named microarchitectural
	side-channel in which it targets hardware infrastructure itself in
	order to exploit information leakage from it. These attacks take advantage
	of performance features that are added to the newer versions of operating
	systems and trick them to reveal sensitive data. Caching and simultaneous
	multithreading (SMT) are two examples of these performance features.
	For example, cache memory is a small component whose goal is to store
	the previous used data with the hope that the data is going to be
	used again soon to increase the efficiency. As a result, with some
	tricks, adversaries may be able to trick the operating system to access
	the cache address and obtain the previous data. Although, disabling
	these efficiency features prevents such attacks, it also significantly
	affects the performance. Hence, other methods should be introduced
	to prevents these attacks without eliminating the aforementioned performance
	features \cite{Micro 1}.
	
	Side channel attacks, based on their impact on the physical structure
	of the targeted circuit, can be categorized into three categories
	of invasive, semi invasive and non invasive attacks. In invasive attacks,
	the physical structure of the target device is altered and cannot
	be returned into its former state after the attack is finished. Moreover,
	these attacks require specialized equipment and direct physical access
	to device's internal components. Although, semi invasive attacks at
	some level modify the physical structure of the devices, they do not
	damage its functionality. Fault injection attacks are categorized
	as semi invasive. Finally, by only monitoring the external leakages
	of the targeted device, without any modification to its physical structure,
	non invasive attacks are performed. Data leakage could be in form
	of power consumption, electromagnetic emission, time differences,
	etc. Since, these attacks do not require direct physical access to
	device's internal components and can be performed remotely, they are
	the easiest and most common types of SCA, however, they are not as
	strong as invasive side channel attacks \cite{PUF- ...}. 
	
	With all being said, there is an important difference between SCA
	on classical cryptography and post-quantum cryptography algorithms.
	The difference is that the underlying mathematics basic of the PQC
	schemes are usually more complex than classical cryptography. In other
	words, in most cases finding the secret key related data in PQC is
	way more harder than classical cryptography which makes SCA analysis
	on PQC more sophisticated \cite{PUF- ...}. 
	
	To prevent SCA, there are basically two types of methods. Those that
	are called generic methods which provide a concrete countermeasure
	without knowing the attack, and custom countermeasures that provide
	security against a specific SCA. There are various techniques that
	are proven to be effective against side-channel attacks. Among them,
	masking, randomizing, blinding, constant time implementation, shielding,
	electromagnetic interference, delay and noise injection, and using
	coherency and redundancy check are the most used techniques. However,
	using these techniques comes with costs. In many cases cost could
	be additional computational overhead, while in some cases it could
	result into design complexity. For example, masking is a generic countermeasure
	which is especially useful in lattice based cryptography to prevent
	power and timing side-channel analysis, imposes heavy overhead upon
	the implementation.
	
	\subsection{attack history/ related work}
	
	\subsubsection*{Dilithium}
	
	In \cite{dilit 1}, by applying power analysis attacks, the authors
	were able to obtain a partial secret key which is then used to successfully
	forge a signature for arbitrary messages. They extended their work
	to include fault attacks in \cite{dilith 2} on the pqm4 software
	implementation of the scheme. Additionally, they proposed a mitigation
	countermeasure to prevent their attack which increases the complexity
	of their attack by $2^{20}$. Further, the work in \cite{dilith 3},
	targeted the pqm4 software implementation of the scheme and provided
	an efficient correlation power analysis attack which could break the
	security of the scheme with only 157 measurements. The work in \cite{dilith 4},
	showed a security weakness to side channel attacks existing in fixed-weight
	polynomial sampling. This is a serious issue as fixed-weight polynomial
	sampling is used in different schemes such as Dilithium, NTRU, and
	NTRU Prime. By targeting the hardware implementation of Dilithium
	on Xilinx Artix-7 FPGA, the work in \cite{dilith 5}, presented a
	detailed analysis on the involved operations of Dilithium that are
	vulnerable against side channel attacks. Moreover, they provided successful
	simple power analysis and correlation power analysis attacks. They
	concluded their paper by providing countermeasures to their attacks.
	By exploiting leakages from bit unpacking procedure of Dilithium,
	Marzougui et al. \cite{dilith 6}, proposed an end-to-end full key
	recovery attack. To test their attack in practice, they mounted it
	on the ARM Cortex-M4 implementation of Dilithium and successfully
	recovered the key by analyzing 756,589 traces. In \cite{Dilith 7},
	a differential fault attack (DFA) is introduced that works on deterministic
	lattice based signature schemes such as Dilithium. They showed that
	a single random fault in signing algorithm is enough to cause key
	recovery through nonce-reuse. Similar to \cite{dilith 6}, the author
	of \cite{Dilith 7} also mounted their attack on the ARM Cortex-M4
	implementation of the scheme. They reported that around 65.2\% of
	execution time of the Dilithium's signature algorithm is unsafe against
	this attack. Finally, the work in \cite{Dilithi C}, reviewed the
	countermeasure techniques that are applicable on lattice based signature
	schemes. In their work, not only did they analyze which types of SCA
	will be prevented by each method, but also provided information on
	how much run time is imposed to implement each one.
	
	\subsubsection*{Kyber}
	
	Side channel analysis of CRYSTALS-Kyber is mainly divided into two
	groups. The first group applies SCA on the software implementation
	of the scheme (mostly on ARM Cortex-M4) while the second group focuses
	on the effects of SCA on the hardware implementation of it. The work
	in \cite{kyber 1 m4}, targeted the Cortex-M4 implementation of various
	PQC schemes including Kyber. In case of Kyber, they showed that by
	using a vulnerability in the decapsulation algorithm and performing
	skipping fault attacks, the secret key can be recovered with only
	a few thousand queries in chosen ciphertext model. Through exploiting
	the leakages of number theoretic transform (NTT) operation, Primas
	et al. \cite{Kyber M4 1.5}, presented a single trace side channel
	attack that is applicable on lattice based encryption schemes. Their
	attack works even on the masked implementation of lattice based encryption
	cryptosystems that use NTT. The authors improved the efficiency of
	their work in \cite{Kyber M4 2}, and performed their attack on the
	ARM Cortex-M4 implementation of Kyber. They showed that by only having
	213 templates, they can successfully retrieve the secret key. By targeting
	KECCAK functions which are widely used in PQC algorithms, the work
	in \cite{Keccak}, showed that the input of these functions can be
	obtained by performing single trace soft analytical side-channel attack
	(SASCA). The impacts of this attack is devastating, as KECCAK functions
	are performed on various sensitive data of PQC schemes such as the
	seed, which is responsible in generation of secret keys. Moreover,
	in \cite{Kyber decod}, a flaw in the message decoding function is
	exploited through electromagnetic side channel attacks and fault injections.
	Furthermore, they showed the practicality of their attack by mounting
	it on the pqm4 implementation of the scheme. Dubrova et al. \cite{Kyber mask}
	proposed a deep-learning message recovery attack that is applicable
	even on the masked implementation of the Kyber. Their attack is capable
	of recovering a message bit on the ARM Cortex-M4 implementation of
	the scheme with probability of more than 99\%.
	
	On the hardware side, the work in \cite{Kyber HW1}, provided a power
	analysis attack on Kyber512 scheme, implemented on Xilinx Virtex-7
	FPGA, and successfully found leakages by using a t-test. In \cite{Kyber HW2},
	the effect of a correlation electromagnetic analysis side channel
	attack on the FPGA implementation of the Kyber512 is investigated.
	By targeting the polynomial multiplication in the decapsulation algorithm,
	they were able to retrieve the secret key by utilizing 166,620 traces.
	The work in \cite{Kyber HW3}, targeted the hardware implementation
	of Kyber768 on Xilinx Artix-7 FPGA and presented a successful profiling
	side channel attack based on deep-learning, that could recover messages
	without requiring the knowledge of any register reference values.
	In \cite{survey kyber-dilithium}, by focusing on a lattice based
	PQC schemes, especially Kyber and Dilithium, a survey of side-channel
	and fault injection attacks is provided. Furthermore, they provided
	countermeasures to the mentioned attacks and implemented them on ARM
	Cortex-M4 and ARM Cortex-A53.
	
	Moreover, various works have been proposed to provide SCA countermeasures
	on Kyber. In \cite{Kyber C1}, a SCA secure binomial sampler is proposed
	that is mountable on lattice based cryptosystems such as NewHope,
	Saber, and Kyber. Their sampler outperformed the state of the art
	in term of imposed overhead. The work in \cite{Kyber C2}, proposed
	the first completely masked implementation of Kyber. They achieved
	it through proposing a high-order bit compression algorithm, and a
	technique to compare uncompressed and compressed polynomials. Compared
	to the reference pqm4 implementation, their implementation reported
	a increase by 3.5 factor in computational overhead. For SCA countermeasures
	on hardware, Kamucheka et al. \cite{Kyber C3} presented a masked
	hardware implementation of Kyber. Their design consists of hiding
	and masking techniques and is useful against simple and differential
	power analysis attacks. By proposing an error detection algorithm
	for NTT operation, Sarker et al. \cite{Kyber C4}, was able to detect
	both transient and permanent faults that could happen in Kyber. Their
	algorithm provided high fault detection rate, while imposing low overhead
	to the scheme. Furthermore, the work in \cite{Kyber C5}, suggested
	to use redundant number representation (RNR) instead of masking to
	prevent side channel attacks. Besides that, they proposed a new Chinese
	remainder theorem based fault detection technique, that could prevent
	fault attacks efficiently. They reported that the Cortex-M4 implementation
	of the combination of these two techniques, requires 1.2x more clock
	cycles compared to the plain implementation. However, by comparing
	their results with masking and redundancy techniques, they provided
	speedup by a factor of 1.3x. 
	
	\subsubsection*{Falcon}
	
	The first electromagnetic side channel analysis of Falcon is presented
	in \cite{Falcon 1st}. Through performing electromagnetic side channel
	attack on the floating-point multiplications, the authors were able
	to successfully obtain the secret key used in signing. The work in
	\cite{falcon 2}, not only presented an improved version of the attack
	in \cite{Falcon 1st} which requires fewer traces and has less complexity,
	but also introduced a new power analysis attack adapting the hidden
	parallelpiped attack, which recovers the secret key. By following
	\cite{falcon 2}, the work in \cite{Falcon 3}, introduced a new power
	analysis attack which significantly reduces the requirement and the
	computational complexity of the attack. 
	
	The first fault attack on the Falcon was introduced in \cite{Falcon fault}.
	This work introduced the initial fault attack against the FALCON signature
	scheme. They employed a technique called basis extraction by aborting
	recursion or zeroing (BEARZ) to carry out this attack. The results
	demonstrated the susceptibility of FALCON to fault attacks on its
	Gaussian sampler, ultimately leading to the disclosure of the private
	key. Moreover, Sarker et al. \cite{Falcon sar}, proposed error detection
	schemes for Saber and FALCON that could detect transient and permanent
	errors with a rate of close to 100\%, while imposing at most 22.59\%,
	19.77\%, and 10.67\% overhead to area, delay, and power, respectively.
	This low overhead increase of their schemes, makes them suitable for
	applications with resource constrained devices.
	
	\subsubsection*{Sphincs+}
	
	Compared to other standardized schemes, little work has been presented
	regarding the side channel analysis of SPHINCS+. Kannwischer et al.
	provided the first systematic side channel analysis on hash based
	signature schemes of XMSS and SPHINCS+ \cite{SPHINCS+ 1 power}. They
	showed that through applying differential power analysis attack, at
	least 32 bit of the secret key of SPHINCS+ can be retrieved. The first
	fault attack on SPHINCS+ is proposed in \cite{SPHIn 1st fault}, in
	which they showed that with only one faulty message they can forge
	any message signature. However, since the computational cost of their
	attack was high, they provided a trade-off to reduce this cost by
	increasing the number of faulty messages. The work in \cite{shpin fault 2},
	provided a practical implementation of \cite{SPHIn 1st fault} on
	Arduino Due board which utilizes ARM Cortex-M3 microprocessor. They
	showed the practicality of the attack's implementation by showing
	how simple can it succeed with only injecting a simple voltage glitch.
	To provide countermeasure for fault attacks, the works in \cite{sphin counter 1,sphin counter 2},
	proposed error detection hash trees that can be applied to stateless
	hash-based signature schemes such as SPHINCS+. Their scheme provides
	fault detection rate of close to 100\% while only adding up to 14.6\%
	overhead on ASIC.
	
	\subsubsection*{BIKE}
	
	BIKE is a KEM scheme that is based on the Niederreiter scheme, but
	instead it is instantiated with QC-MDPC codes. By finding a flaw in
	the decryption algorithm, Guo et al. \cite{BIKE 1}, proposed a key
	recovery attack that could retrieve the key in matter of several minutes.
	They took advantage of the dependency between the secret key and a
	failure procedure that could happen in decoding. By improving the
	work in \cite{BIKE 1}, in 2018, Nilson et al. proposed a new attack
	that only utilizes a single error vector \cite{BIKE 2}. This error
	vector then leads to a decoding failure which will be then used for
	key recovery. Further, the work in \cite{BIKE 3- FO} found a leakage
	occurring in the Fujisaki-Okamoto transformation that is used in Kyber,
	HQC and BIKE schemes. The leakage happens in the re-encryption step
	in the decapsulation algorithm because of the PRF execution. Furthermore,
	by analyzing the execution time differences of rejection sampling
	algorithm on altered and unaltered versions of the input message,
	Guo et al. \cite{BIKE 4} proposed two new attacks that could successfully
	retrieve the secret key of BIKE and HQC schemes. The work in \cite{BIKE 5},
	proposed a multiple trace and a single track attack which can successfully
	recover secret indices and work even on ephemeral keys. By applying
	their attack on BIKE and LEDAcrypt, they pinpointed their vulnerabilities
	of these two schemes. However, these attacks can be prevented through
	randomization, hiding and masking techniques. 
	
	\subsubsection*{McEliece}
	
	Since, McEliece has been first proposed in 1978 {[}XXX{]}, it has
	been studied more compared to other schemes. By targeting the software
	implementation of McEliece scheme on FlexiProvider platform, Strenzke
	et al. \cite{McEliece 1} introduced a timing attack that could successfully
	break the security of the cryptosystem. They concluded their work
	by presenting countermeasures to their attack. The work in \cite{Mc -2},
	presented a timing attack on the Patterson algorithm that is used
	for efficient decoding of Goppa codes. Since, McEliece cryptosystem
	uses Goppa codes for encoding and decoding, they applied it to a FPGA
	implementation of the McEliece cryptosystem directly, and showed serious
	vulnerabilities of the cryptosystem. Similarly, the work in \cite{Mc 2.5},
	found a vulnerability in the Patterson algorithm which could utilized
	through a timing attack to reduce the search space of the secret key
	of the McEliece cryptosystem against brute force attack drastically.
	By continuing the work in \cite{Mc -2}, in \cite{Mc 3} an electromagnetic
	side channel attack is proposed and tested on FPGA implementation
	of the system. By using a technique they called iterative column chunking
	they were able to reduce the number of required measurements. Further,
	they showed that with only about 560 measurements, the plaintext could
	be recovered. Besides the mentioned timing attacks, the works in \cite{Mc PA 1,Mc PA 2}
	applied power analysis attack to McEliece scheme and investigated
	its effects. More specifically, in \cite{Mc PA 1} a simple power
	analysis attack is proposed that exploits the dependency between the
	number of iteration in Paterson algorithm and error vector weight.
	By applying this attack on the FPGA implementation of the scheme,
	they showed that the error vector could be obtained with little overhead.
	Moreover, by applying power analysis attack on both FPGA and ARM implementation
	of McEliece, Guo et al. \cite{Mc PA 2}, presented a key recovery
	attack that could fully retrieve the key by gathering about 800 traces
	and performing a machine-learning-based classification algorithm on
	them. Furthermore, through combining machine learning with side channel
	attacks, Colombier et al. \cite{Mc pa 3}proposed a new power analysis
	attack that exploits the leakage from matrix-vector multiplication
	operation which could eventually recover the plaintext efficiently. 
	
	Through the years, various works have been dedicated to provide side-channel
	countermeasures to implementations of the McEliece. The work in \cite{MC count 1},
	presented a countermeasure against power analysis side channel attack
	on the Cortex-M3 software implementation of the McEliece cryptosystem.
	The works in \cite{MC fault 1,MC fault 2}, focused on the fault detection
	aspects of McEliece cryptosystem. By targeting the finite field multiplier,
	the authors proposed natural and injected fault detection schemes
	that provide 100\% detection rate on the FPGA implementation of the
	cryptosystem. Moreover, Cintas-Canto et al. \cite{MC fault 3}, proposed
	efficient fault detection constructions that could be applied to code
	based cryptosystems. They applied their schemes on McEliece cryptosystem
	and implemented it on the Kintex-7 FPGA device. Their implementation
	results indicate a 100\% error detection rate while adding 49\% overhead
	to area and delay, at the worst case scenario.
	
	\subsubsection*{HQC}
	
	Since, HQC shares similar operations and architectures with other
	cryptosystesm such as BIKE, many of the previous works are also applicable
	to HQC. For example, we mentioned earlier that the work in \cite{BIKE 3- FO}
	found a leakage in the Fujisaki-Okamoto transformation that transforms
	any CPA-PKE scheme into a CCA-KEM scheme. Since HQC uses this transformation,
	it is also vulnerable to the attack in \cite{BIKE 3- FO}. Besides
	that, recently Huang et al. \cite{HQC 1}, proposed the first chosen-ciphertext
	cache-timing attack on the reference implementation of the HQC cryptosystem.
	They exploited a vulnerability in the vector generation process of
	the reference implementation of HQC and practically recovered the
	secret key. Moreover, the first power analysis side channel on HQC
	is presented in \cite{HQC 2}. Their attack requires chosen-ciphertext
	access model and based on the mounted decoding algorithm on the scheme,
	it makes the queries in a way to efficiently retrieve a large part
	of the secret key. They showed that their attack is successful on
	the ARM Cortex-M4 implementation of the scheme requiring less than
	10000 measurements. Similarly, in \cite{HQC 3} a chosen-ciphertext
	key recovery side channel attack is proposed that exploits the static
	secret key reuse feature of the micro controller. By taking advantage
	of the leakages of the diffusion property of the Reed-Muller decoding
	step, they were able to retrieve the whole secret key. To test their
	attack in practice, they mounted it on the Cortex-M4 microprocessor
	and were able to obtain the whole secret key with 19200 electromagnetic
	traces. In \cite{HQC 4}, a horizontal attack is introduced which
	targets the Reed-Solomon decoding algorithm of HQC. Although not breaking
	the security of the scheme completely, the authors showed that $2^{96}$
	operations are needed to successfully attack the scheme which is in
	contrast to the $2^{128}$ claimed security level of HQC. They concluded
	their paper by proposing a shuffling countermeasure to prevent their
	attack. Moreover, Schamberger et al. \cite{HQC 5}, proposed a new
	side channel attack that is applicable on the third version of the
	HQC scheme. Their attack uses the leakages of the Reed-Solomon decoder
	and SHAKE256 hash function and outperforms the state of the art by
	the factor of 12 in term of number of required queries. 


==> acmart-primary/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> acmart-primary/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

